Selection on $X_1+X_2+\cdots + X_m$ with layer-ordered heaps

Selection on $X_1+X_2+\cdots + X_m$ is an important problem with many applications in areas such as max-convolution, max-product Bayesian inference, calculating most probable isotopes, and computing non-parametric test statistics, among others. Faster-than-na\"{i}ve approaches exist for $m=2$: Frederickson (1993) published the optimal algorithm with runtime $O(k)$ and Kaplan \emph{et al.} (2018) has since published a much simpler algorithm which makes use of Chazelle's soft heaps (2003). No fast methods exist for $m>2$. Johnson \& Mizoguchi (1978) introduced a method to compute the single $k^{th}$ value when $m>2$, but that method runs in $O(m\cdot n^{\lceil\frac{m}{2}\rceil} \log(n))$ time and is inefficient when $m \gg 1$ and $k \ll n^{\lceil\frac{m}{2}\rceil}$. In this paper, we introduce the first efficient methods, both in theory and practice, for problems with $m>2$. We introduce the ``layer-ordered heap,'' a simple special class of heap with which we produce a new, fast selection algorithm on the Cartesian product. Using this new algorithm to perform $k$-selection on the Cartesian product of $m$ arrays of length $n$ has runtime $\in o(k\cdot m)$. We also provide implementations of the algorithms proposed and evaluate their performance in practice.

==> figs/depths-visited-on-sort-tree.tex <==

\begin{table}
\caption{Varying K with an Exponential Dist & Vary k & root to leaves}

\begin{tabular}{ r l l l l l l }
64   & 33.50  & 18.20 & 10.62 & 6.812 & 4.875 & 3.900 \\
128  & 65.50  & 34.20 & 18.62 & 10.75 & 6.843 & 4.890 \\
512  & 257.5  & 130.2 & 66.62 & 34.81 & 18.87 & 10.89 \\
1024 & 513.5  & 258.2 & 130.6 & 66.68 & 34.84 & 18.82 \\
2048 & 1025.0 & 502.7 & 252.9 & 66.18 & 34.59 & 18.70 \\
\end{tabular}
\end{table}

\begin{table}
\caption{Varying $k$ with Uniform distribution}
\begin{tabular}{ r l l l l l l }
64   & 15.50 & 6.000  & 3.750 & 3.312 & 3.031 & 2.953\\
128  & 52.50 & 11.250 & 6.875 & 3.562 & 3.12  & 3.031\\
512  & 62.00 & 14.250 & 6.375 & 4.25 & 3.312  & 3.046\\
1024 & 76.50 & 13.250 & 6.125 & 3.937 & 3.218 & 2.984\\
2048 & 471.0 & 42.000 & 9.125 & 4.75 & 3.375  & 3.109\\

\end{tabular}
\end{table}

\begin{table}
\caption{Varying $m$ with exponential distribution all with $k$ = 512 and $n$ = 1024}
\begin{tabular}{ r l l l l l l l l l l l l }

64   & 1024.0 & 139.5 & 19.50  & 7.125 & 4.062 & 3.312 & 3.03 \\
128  & 512.0  & 257.5 & 130.3  & 66.63 & 34.81 & 18.91 & 10.93 \\
256  & 512.0  & 257.5 & 130.3  & 66.63 & 34.75 & 18.81 & 10.87 & 6.914 \\
512  & 512.0  & 257.5 & 130.3  & 66.63 & 34.75 & 18.84 & 10.87 & 6.906 & 4.914 & 3.914 \\
1024 & 512.0  & 257.5 & 130.3  & 66.63 & 34.81 & 18.88 & 10.90 & 6.914 & 4.902 & 3.919 & 3.418 \\
2048 & 512.0  & 46.50 & 10.75  & 4.630 & 3.500 & 3.156 & 3.046 & 2.960 & 2.929 & 2.927 & 2.920 & 2.912 \\

\end{tabular}
\end{table}

\begin{table}
\caption{ Varying $m$ with uniform distribution, all with $k = 512$$ and $n = 1024$$  }
\begin{tabular}{ r l l l l l l l l l l l l }

64   & 512.0 & 49.00 & 12.00 & 5.625 & 3.813 & 3.3434 & 3.125 \\
128  & 512.0 & 48.50 & 10.75 & 5.500 & 3.813 & 3.281 & 3.078 & 2.961 \\ 
256  & 512.0 & 54.50 & 12.00 & 5.500 & 3.688 & 3.250 & 3.078  & 2.992  & 2.945 \\
512  & 512.0 & 71.00 & 14.50 & 6.000 & 4.125 & 3.281 & 3.109 & 2.977 & 2.945 & 2.928 \\
1024 & 512.0 & 45.50 & 14.25 & 5.875 & 4.063 & 3.313 & 3.094 & 2.961 & 2.938 & 2.930 & 2.913 \\
2048 & 512.0 & 46.50 & 10.75 & 4.625 & 3.500 & 3.156 & 3.047 & 2.961 & 2.930 & 2.928 & 2.921 & 2.913 \\

\end{tabular}
\end{table}

